System description: Isabelle/jEdit in 2014

This is an updated system description for Isabelle/jEdit, according to the official release Isabelle2014 (August 2014). The following new PIDE concepts are explained: asynchronous print functions and document overlays, syntactic and semantic completion, editor navigation, management of auxiliary files within the document-model.

==> eptcsdata.tex <==
\providecommand{\firstpage}{84}
\providecommand{\publicationstatus}{C. Benzm\"uller and B. Woltzenlogel Paleo (Eds.):\\ 
Eleventh Workshop on User Interfaces for Theorem Provers (UITP 2014)\\
EPTCS 167, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.167.10}{10.4204/EPTCS.167.10}}
\pdfoutput=1

